LLMs in Cloud: A Discussion on Architecture, Orchestration, and Inference

The widespread deployment of foundational Large Language Models (LLM) across cloud datacenters marks a fundamental paradigm shift from stateless deep learning toward distributed, memory-intensive generative workloads. However, serving massive foundation models under stringent Service Level Objectives (SLO) exposes critical physical and system bottlenecks. These challenges include the persistent High Bandwidth Memory (HBM) wall, operational asymmetry between compute-bound prefilling and memory-bandwidth-bound decoding, explosive Key-Value (KV) cache expansion, prohibitive serverless cold starts, and hardware reliability vulnerabilities. Existing literature reviews remain layer-siloed, decoupling low-level accelerator virtualization from cluster orchestration and runtime inference, while largely overlooking defining advancements from 2024 to 2026. To address these limitations, this study presents a comprehensive, cross-layer systematic review guided by the Preferred Reporting Items for Systematic Reviews and Meta-Analyses (PRISMA) 2020 framework. We synthesize a holistic taxonomy unifying hardware virtualization, cluster-level scheduling, and runtime inference optimizations, including iteration-level continuous batching, prefill-decoding disaggregation, and hierarchical KV cache offloading. Furthermore, we evaluate resilient cloud-native service architectures, examining scale-to-zero serverless paradigms, fault-tolerant checkpointing against silent data corruption, and hardware-enforced Trusted Execution Environments (TEEs) for multi-tenant isolation. Finally, we formalize the multi-dimensional Pareto trade-offs governing throughput, latency, monetary cost, and confidentiality, outlining a forward-looking research roadmap spanning Compute Express Link (CXL) memory pooling, in-memory computing, and autonomous multi-agent control planes to guide future cloud LLM infrastructure.

==> Utils/acronyms.tex <==
% Credits to @LofiTurtle
% Setting up lightweight high-performance acronym engine (100% compatible with acro syntax)
\usepackage{keyval}

\makeatletter
% Define lightweight parser keys
\define@key{acrodecl}{short}{\def\@acro@short{#1}}
\define@key{acrodecl}{long}{\def\@acro@long{#1}}
\define@key{acrodecl}{short-plural}{\def\@acro@shortp{#1}}
\define@key{acrodecl}{long-plural}{\def\@acro@longp{#1}}

\newcommand{\DeclareAcronym}[2]{%
  \def\@acro@short{#1}%
  \def\@acro@long{#1}%
  \def\@acro@shortp{}%
  \def\@acro@longp{}%
  \setkeys{acrodecl}{#2}%
  \ifx\@acro@shortp\@empty
    \edef\@acro@shortp{\unexpanded\expandafter{\@acro@short}s}%
  \fi
  \ifx\@acro@longp\@empty
    \edef\@acro@longp{\unexpanded\expandafter{\@acro@long}s}%
  \fi
  \expandafter\xdef\csname acro@short@#1\endcsname{\unexpanded\expandafter{\@acro@short}}%
  \expandafter\xdef\csname acro@long@#1\endcsname{\unexpanded\expandafter{\@acro@long}}%
  \expandafter\xdef\csname acro@shortp@#1\endcsname{\unexpanded\expandafter{\@acro@shortp}}%
  \expandafter\xdef\csname acro@longp@#1\endcsname{\unexpanded\expandafter{\@acro@longp}}%
  \ifx\@acro@list\@empty
    \gdef\@acro@list{#1}%
  \else
    \g@addto@macro\@acro@list{,#1}%
  \fi
}
\def\@acro@list{}

% \ac and \acp with automatic first-use long form expansion
\NewDocumentCommand{\ac}{s m}{%
  \expandafter\ifcsname acro@short@#2\endcsname
    \expandafter\ifx\csname acro@used@#2\endcsname\relax
      \IfBooleanF{#1}{\expandafter\gdef\csname acro@used@#2\endcsname{1}}%
      \csname acro@long@#2\endcsname\space(\csname acro@short@#2\endcsname)%
    \else
      \csname acro@short@#2\endcsname
    \fi
  \else
    \textbf{#2}%
  \fi
}

\NewDocumentCommand{\acp}{s m}{%
  \expandafter\ifcsname acro@shortp@#2\endcsname
    \expandafter\ifx\csname acro@used@#2\endcsname\relax
      \IfBooleanF{#1}{\expandafter\gdef\csname acro@used@#2\endcsname{1}}%
      \csname acro@longp@#2\endcsname\space(\csname acro@shortp@#2\endcsname)%
    \else
      \csname acro@shortp@#2\endcsname
    \fi
  \else
    \textbf{#2s}%
  \fi
}

\NewDocumentCommand{\acs}{s m}{%
  \expandafter\ifcsname acro@short@#2\endcsname
    \csname acro@short@#2\endcsname
  \else
    \textbf{#2}%
  \fi
}

\NewDocumentCommand{\acl}{s m}{%
  \expandafter\ifcsname acro@long@#2\endcsname
    \csname acro@long@#2\endcsname
  \else
    \textbf{#2}%
  \fi
}

\NewDocumentCommand{\acresetall}{}{%
  \@for\@key:=\@acro@list\do{%
    \expandafter\global\expandafter\let\csname acro@used@\@key\endcsname\relax
  }%
}

% Compatibility no-ops for acro setup
\NewDocumentCommand{\acsetup}{m}{}
\NewDocumentCommand{\NewAcroTemplate}{O{} m +m}{}

% Two-column List of Acronyms rendering matching template
\NewDocumentCommand{\printacronyms}{O{}}{%
  \section*{List of Acronyms}%
  \begingroup\scriptsize\raggedright
  \begin{multicols}{2}
    \@for\@key:=\@acro@list\do{%
      \noindent\hangindent=2.2cm\hangafter=1
      \makebox[2.2cm][l]{\textbf{\csname acro@short@\@key\endcsname}}%
      \csname acro@long@\@key\endcsname\par\vspace{1.5pt}
    }
  \end{multicols}
  \endgroup
}
\makeatother


% Declaring comprehensive acronyms here

\DeclareAcronym{ABFT}{
    short = ABFT,
    long  = Algorithm-Based Fault Tolerance
}

\DeclareAcronym{AI}{
    short = AI,
    long  = Artificial Intelligence
}

\DeclareAcronym{AIOps}{
    short = AIOps,
    long  = Artificial Intelligence for IT Operations
}

\DeclareAcronym{AMX}{
    short = AMX,
    long  = Advanced Matrix Extensions
}

\DeclareAcronym{API}{
    short = API,
    long  = Application Programming Interface
}

\DeclareAcronym{ASIC}{
    short = ASIC,
    long  = Application-Specific Integrated Circuit
}

\DeclareAcronym{AWS}{
    short = AWS,
    long  = Amazon Web Services
}

\DeclareAcronym{AYCI}{
    short = AYCI,
    long  = All-You-Can-Inference
}

\DeclareAcronym{BiSR}{
    short = BiSR,
    long  = Bidirectional Semi-white-box Reconstruction
}

\DeclareAcronym{CCA}{
    short = CCA,
    long  = Confidential Compute Architecture
}

\DeclareAcronym{CoVe}{
    short = CoVe,
    long  = Chain-of-Verification
}

\DeclareAcronym{CPU}{
    short = CPU,
    long  = Central Processing Unit
}

\DeclareAcronym{CUDA}{
    short = CUDA,
    long  = Compute Unified Device Architecture
}

\DeclareAcronym{CXL}{
    short = CXL,
    long  = Compute Express Link
}

\DeclareAcronym{DDoS}{
    short = DDoS,
    long  = Distributed Denial-of-Service
}

\DeclareAcronym{DL}{
    short = DL,
    long  = Deep Learning
}

\DeclareAcronym{DLIS}{
    short = DLIS,
    long  = Deep Learning Inference service
}

\DeclareAcronym{DMA}{
    short = DMA,
    long  = Direct Memory Access
}

\DeclareAcronym{DNN}{
    short = DNN,
    long  = Deep Neural Net
}

\DeclareAcronym{DOI}{
    short = DOI,
    long  = Digital Object Identifier
}

\DeclareAcronym{DRAM}{
    short = DRAM,
    long  = Dynamic Random Access Memory
}

\DeclareAcronym{DRL}{
    short = DRL,
    long  = Deep Reinforcement Learning
}

\DeclareAcronym{DSE}{
    short = DSE,
    long  = Design Space Exploration
}

\DeclareAcronym{DVFS}{
    short = DVFS,
    long  = Dynamic Voltage and Frequency Scaling
}

\DeclareAcronym{FaaS}{
    short = FaaS,
    long  = Function-as-a-Service
}

\DeclareAcronym{FHE}{
    short = FHE,
    long  = Fully Homomorphic Encryption
}

\DeclareAcronym{FP16}{
    short = FP16,
    long  = 16-bit Floating-Point
}

\DeclareAcronym{FPGA}{
    short = FPGA,
    long  = Field Programmable Gate Array
}

\DeclareAcronym{FRAM}{
    short = FRAM,
    long  = Functional Resonance Analysis Method
}

\DeclareAcronym{GPU}{
    short = GPU,
    long  = Graphics Processing Unit
}

\DeclareAcronym{HBM}{
    short = HBM,
    long  = High Bandwidth Memory
}

\DeclareAcronym{HDC}{
    short = HDC,
    long  = Hyperdimensional Computing
}

\DeclareAcronym{HIP}{
    short = HIP,
    long  = Hierarchical Imprecise Probability
}

\DeclareAcronym{HPA}{
    short = HPA,
    long  = Horizontal Pod Autoscaler
}

\DeclareAcronym{IO}{
    short = IO,
    long  = Input/Output
}

\DeclareAcronym{ITL}{
    short = ITL,
    long  = Inter-Token Latency
}

\DeclareAcronym{K8s}{
    short = K8s,
    long  = Kubernetes
}

\DeclareAcronym{KISim}{
    short = KISim,
    long  = Kubernetes Inference Simulator
}

\DeclareAcronym{KV}{
    short = KV,
    long  = Key-Value
}

\DeclareAcronym{LightGBM}{
    short = LightGBM,
    long  = Light Gradient-Boosting Machine
}

\DeclareAcronym{LLM}{
    short = LLM,
    long  = Large Language Model
}

\DeclareAcronym{LoRA}{
    short = LoRA,
    long  = Low-Rank Adaptation
}

\DeclareAcronym{LSH}{
    short = LSH,
    long  = Locality-Sensitive Hashing
}

\DeclareAcronym{LSTM}{
    short = LSTM,
    long  = Long Short-Term Memory
}

\DeclareAcronym{MAS}{
    short = MAS,
    long  = Multi-Agent System
}

\DeclareAcronym{MEC}{
    short = MEC,
    long  = Multi-access Edge Computing
}

\DeclareAcronym{MIG}{
    short = MIG,
    long  = Multi-Instance GPU
}

\DeclareAcronym{MLaaS}{
    short = MLaaS,
    long  = Machine Learning as a Service
}

\DeclareAcronym{MLSys}{
    short = MLSys,
    long  = Machine-Learning Systems
}

\DeclareAcronym{MPS}{
    short = MPS,
    long  = Multi-Process Service
}

\DeclareAcronym{MTTR}{
    short = MTTR,
    long  = Mean Time To Recovery
}

\DeclareAcronym{NIC}{
    short = NIC,
    long  = Network Interface Card
}

\DeclareAcronym{NPU}{
    short = NPU,
    long  = Neural Processing Unit
}

\DeclareAcronym{NVLink}{
    short = NVLink,
    long  = NVIDIA Link
}

\DeclareAcronym{OOM}{
    short = OOM,
    long  = Out-Of-Memory
}

\DeclareAcronym{P-LoRA}{
    short = P-LoRA,
    long  = Predictive-LoRA
}

\DeclareAcronym{PCIe}{
    short = PCIe,
    long  = Peripheral Component Interconnect Express
}

\DeclareAcronym{PHPA}{
    short = PHPA,
    long  = Predictive Horizontal Pod Autoscaling
}

\DeclareAcronym{PipeCast}{
    short = PipeCast,
    long  = Pipelined Multicast Inference
}

\DeclareAcronym{PISeL}{
    short = PISeL,
    long  = Pipelining DNN Inference for Serverless
}

\DeclareAcronym{PP}{
    short = PP,
    long  = Pipeline Parallelism
}

\DeclareAcronym{PPO}{
    short = PPO,
    long  = Proximal Policy Optimization
}

\DeclareAcronym{PRISMA}{
    short = PRISMA,
    long  = Preferred Reporting Items for Systematic Reviews and Meta-Analyses
}

\DeclareAcronym{QoS}{
    short = QoS,
    long  = Quality of Service
}

\DeclareAcronym{RAG}{
    short = RAG,
    long  = Retrieval-Augmented Generation
}

\DeclareAcronym{RAM}{
    short = RAM,
    long  = Random Access Memory
}

\DeclareAcronym{RCA}{
    short = RCA,
    long  = Root Cause Analysis
}

\DeclareAcronym{RDMA}{
    short = RDMA,
    long  = Remote Direct Memory Access
}

\DeclareAcronym{RoCE}{
    short = RoCE,
    long  = RDMA over Converged Ethernet
}

\DeclareAcronym{RQ}{
    short = RQ,
    long  = Research Question
}

\DeclareAcronym{SDC}{
    short = SDC,
    long  = Silent Data Corruption
}

\DeclareAcronym{SDN}{
    short = SDN,
    long  = Software-Defined Networking
}

\DeclareAcronym{SEV}{
    short = SEV,
    long  = Secure Encrypted Virtualization
}

\DeclareAcronym{SGX}{
    short = SGX,
    long  = Software Guard Extensions
}

\DeclareAcronym{SLA}{
    short = SLA,
    long  = Service Level Agreement
}

\DeclareAcronym{SLM}{
    short = SLM,
    long  = Small Language Model
}

\DeclareAcronym{SLO}{
    short = SLO,
    long  = Service Level Objective
}

\DeclareAcronym{SLR}{
    short = SLR,
    long  = Systematic Literature Review
}

\DeclareAcronym{SM}{
    short = SM,
    long  = Streaming Multiprocessor
}

\DeclareAcronym{SMS}{
    short = SMS,
    long  = Stateful Microservices
}

\DeclareAcronym{SOP}{
    short = SOP,
    long  = Standard Operating Procedure
}

\DeclareAcronym{SPMD}{
    short = SPMD,
    long  = Single Program Multiple Data
}

\DeclareAcronym{SSD}{
    short = SSD,
    long  = Solid-State Drive
}

\DeclareAcronym{STPA}{
    short = STPA,
    long  = System-Theoretic Process Analysis
}

\DeclareAcronym{TBT}{
    short = TBT,
    long  = Time-Between-Tokens
}

\DeclareAcronym{TDX}{
    short = TDX,
    long  = Trust Domain Extensions
}

\DeclareAcronym{TEE}{
    short = TEE,
    long  = Trusted Execution Environment
}

\DeclareAcronym{TP}{
    short = TP,
    long  = Tensor Parallelism
}

\DeclareAcronym{TPU}{
    short = TPU,
    long  = Tensor Processing Unit
}

\DeclareAcronym{TTFT}{
    short = TTFT,
    long  = Time-To-First-Token
}

\DeclareAcronym{TVM}{
    short = TVM,
    long  = Tensor Virtual Machine
}

\DeclareAcronym{URL}{
    short = URL,
    long  = Uniform Resource Locator
}

\DeclareAcronym{V-and-V}{
    short = V\&V,
    long  = Verification and Validation
}

\DeclareAcronym{vLLM}{
    short = vLLM,
    long  = virtual Large Language Model
}

\DeclareAcronym{VM}{
    short = VM,
    long  = Virtual Machine
}

\DeclareAcronym{VSA}{
    short = VSA,
    long  = Vector Symbolic Architecture
}

